Efficient Data Management for Intelligent Urban Mobility Systems

Modern intelligent urban mobility applications are underpinned by large-scale, multivariate, spatiotemporal data streams. Working with this data presents unique challenges of data management, processing and presentation that is often overlooked by researchers. Therefore, in this work we present an integrated data management and processing framework for intelligent urban mobility systems currently in use by our partner transit agencies. We discuss the available data sources and outline our cloud-centric data management and stream processing architecture built upon open-source publish-subscribe and NoSQL data stores. We then describe our data-integrity monitoring methods. We then present a set of visualization dashboards designed for our transit agency partners. Lastly, we discuss how these tools are currently being used for AI-driven urban mobility applications that use these tools.

==> LaTeX/figures/energy_predictor.tex <==
\begin{figure}[t]
\centering

\includegraphics[width=0.9\columnwidth]{LaTeX/images/energy_predictor.png}
\caption{TODO}
\label{fig: energy predictor}


\end{figure}

==> LaTeX/figures/occupancy.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}{0.9\columnwidth}
    \includegraphics[width=\textwidth]{LaTeX/images/ridershipgraph.png}
    \caption{}
    \label{subfig: occupancy graph}
\end{subfigure}
\begin{subfigure}{0.9\columnwidth}
    \includegraphics[width=\textwidth]{LaTeX/images/ridershiproute.png}
    \caption{}
    \label{subfig: occupancy route}
\end{subfigure}
\caption{Occupancy visualization dashboard: (a) mean occupancy per route from January 1, 2020 to May 1, 2020. (b) distribution of maximum average occupancy per route from January 1, 2020 to May 1, 2020.}
\label{fig: occupancy dashboard}
\vspace{-0.2in}
\end{figure}
